Adversarial Environment Generation for Learning to Navigate the Web

Learning to autonomously navigate the web is a difficult sequential decision making task. The state and action spaces are large and combinatorial in nature, and websites are dynamic environments consisting of several pages. One of the bottlenecks of training web navigation agents is providing a learnable curriculum of training environments that can cover the large variety of real-world websites. Therefore, we propose using Adversarial Environment Generation (AEG) to generate challenging web environments in which to train reinforcement learning (RL) agents. We provide a new benchmarking environment, gMiniWoB, which enables an RL adversary to use compositional primitives to learn to generate arbitrarily complex websites. To train the adversary, we propose a new technique for maximizing regret using the difference in the scores obtained by a pair of navigator agents. Our results show that our approach significantly outperforms prior methods for minimax regret AEG. The regret objective trains the adversary to design a curriculum of environments that are "just-the-right-challenge" for the navigator agents; our results show that over time, the adversary learns to generate increasingly complex web navigation tasks. The navigator agents trained with our technique learn to complete challenging, high-dimensional web navigation tasks, such as form filling, booking a flight etc. We show that the navigator agent trained with our proposed Flexible b-PAIRED technique significantly outperforms competitive automatic curriculum generation baselines -- including a state-of-the-art RL web navigation approach -- on a set of challenging unseen test environments, and achieves more than 80% success rate on some tasks.

==> WebDesignPAIRED (DeepRL Workshop) (Arxiv)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> WebDesignPAIRED (DeepRL Workshop) (Arxiv)/src/background.tex <==
\section{Background}

\subsection{Web Navigation Problem}

Following previous work \citep{shi2017world,gur2018learning,liu2018reinforcement}, we formulate web navigation as a sequential decision making problem where we train an agent, parameterized by a network $\pi(a_t | s_t; \Theta_i)$, that maps an input state $s_t$ to output actions $a_t$ to maximize the cumulative discounted reward, .i.e.,  $O=\sum_{t=0}^{T}{\gamma^t r_t}$ where $r_t$ is the reward at time step $t$, $\gamma$ is a discount factor, and $T$ is the length of an episode.
We use the web page and user instruction as the input state. The web page is dynamically updated at each time step, while the instruction is fixed at the beginning of an episode.
We represent web pages using Document Object Model (DOM), a tree of elements in a page, where each element is denoted by a set of (attribute, value) pairs and an array of features (such as spatial coordinates).
Instructions are given as a set of fields where each field is a (key, value) pair.
Keys are fixed for each task and values dynamically change based on user input.

Each action is represented as a tuple (element, field) that denotes acting on the element using the field as an input; i.e. typing the value of the field into the element.
Agents receive a task success reward (1.0 or -1.0) at the end of each episode, a potential-based reward when the value of an element in the page is updated, and a small penalty each timestep to encourage efficient navigation.
As an example, consider a flight booking task where the agent is given an instruction \{\texttt{"Departure Date": "Friday", Destination Airport: "Los Angeles (LAX)"}\}.
The agent first picks a field (e.g. destination airport) and finds the corresponding text box in the page; then the corresponding value (``Los Angeles (LAX)") typed in to the text box.
If this value is correct, the agent receives a positive reward of $1 /  N $ where $N$ is the number of fields.

\subsection{Protagonist Antagonist Induced Regret Environment Design (PAIRED)}
Adversarial Environment Generation (AEG) trains an adversary policy $\pi_E$ to design environments to minimize the performance of an agent's policy, $\pi_P$. Let $R^P_i = \sum_{t=1}^T\gamma^tr_t^P$ be the total reward received by the agent for trajectory $i$. In minimax AEG, the objective for the adversary is simply: $-R^P$. Thus, minimax adversaries are incentivized to create excessively difficult or impossible environments, which may not enable the agent to learn. Instead, PAIRED \citep{dennis2020emergent} trains the adversary to maximize the agent's \textit{regret}, which is defined as the difference between the agent's return and the return of the optimal policy, $R^*-R^P$. When the reward function includes an incentive to complete the task more efficiently (which is true in our case), the regret will be highest for easy tasks which could be completed in a few steps by the optimal policy, but which the current policy fails to complete. Therefore, an adversary that maximizes the regret will continue to propose easier tasks until the agent begins to solve them, making regret a desirable objective for AEG.

To estimate the regret, PAIRED
introduces a third agent, the \textit{antagonist} (with policy $\pi_A$), and  constrains the adversary to only generate feasible environments which the antagonist can complete. 
When the adversary generates an environment $E$, both the protagonist and antagonist collect $M$ trajectories with returns $R^P_{1},...,R^P_{M}, R^A_{1},...,R^A_{M}$ in $E$. The regret is then estimated as:
\begin{align}
    \textsc{Regret} = \max_i R^A_i - \frac{1}{M}\sum_{m=1}^M R^P_m
    \label{eq:paired_regret}
\end{align}

As \citet{dennis2020emergent} show, if the adversary and antagonist coordinate and reach a Nash equilibrium with the protagonist, then the protagonist will have learned to minimize the regret. However, in practice gradient-based multi-agent RL has no convergence guarantees, is highly non-stationary, and will often fail to converge \citep{mazumdar2019policy,mazumdar2019finding}. If the antagonist and adversary in PAIRED fail to coordinate, then PAIRED minimizes regret with respect to the antagonist's policy. In that case, the objective in Equation \ref{eq:paired_regret} only forces the protagonist to learn to be as good as the antagonist. If the antagonist fails to improve, or reaches a local optimum, then the adversary cannot continue to train the protagonist. In Section \ref{sec:flexible} we propose an improved objective which addresses this problem. 

==> WebDesignPAIRED (DeepRL Workshop) (Arxiv)/src/conclusion.tex <==
\vspace*{-0.1in}
\section{Conclusion}
\vspace*{-0.1in}
This work presents a novel technique for Adversarial Environment Generation (AEG), which we show improves significantly over prior work. In addition, we apply AEG to the problem of web navigation, and provide an open-source environment that enables learning to design complex websites out of a set of compositional primitives. Our \WEDPb\ method is able to generate a curriculum of increasingly complicated websites, and successfully trains agents which can navigate challenging, high-dimensional websites. 

==> WebDesignPAIRED (DeepRL Workshop) (Arxiv)/src/experiments.tex <==
\section{Experiments and Methods}
We evaluate our models on a variety of web environments implemented in MiniWoB framework \citep{shi2017world,liu2018reinforcement}.
We implemented several challenging websites with varying difficulty levels using the same set of design primitives.
These environments include `Login', `Enter Address', `Flight Booking', `Enter Payment', and `Shopping' websites, where the agents need to enter text or select information in the website while navigating between pages.
Each environment comes with 4 different difficulty levels by gradually adding more primitives to websites.
These environments are never explicitly presented to agents during training, so performance in them measures how well agents can generalize to unseen websites at test time.

\textbf{Agent architecture:} Following \citet{gur2018learning}, we utilize an LSTM based DOM tree encoder and a feed forward network to encode profile fields.
The \webnav\ agent policy outputs a joint distribution over elements and fields by measuring pairwise similarities between element encodings and profile fields.
We compute the state-value by using the marginal distribution of elements as attention weights over element encodings and passing the context vector through a FF network.
Web navigation agents are trained with an actor-critic algorithm \citep{liu2018reinforcement}.
We train the LSTM-based adversary network using \WEDP\ and \WEDPb\ with policy gradient.

\textbf{Baselines:} We benchmark PAIRED, \WEDP, and \WEDPb\ against two additional baselines. First, a Domain Randomization (DR) agent, which we implement using a similar approach as \citet{dennis2020emergent}.
We first sample the number of empty pages $k$ from a uniform distribution $U[0,K]$.
Next, we randomly sample a primitive (including SKIP), and a page from $U[0,k]$ for $N$ steps.
Second, a Curriculum Learning (CL) approach, which adapts the scheduled curriculum idea of \citet{gur2018learning} to zero-shot environment generation where we are not given a specific website but a set of design primitives.
We randomly sample each primitive w.r.t. a probability $p$ where $p$ is initialized with a small number and scheduled to reach $1.0$ during training.

\section{Results}
\begin{figure}[tb]
\small
\centering
\vspace{-.7cm}
    \subfloat[Login]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/login.png}
    }%
    \subfloat[Address]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/address.png}
    }%
    \subfloat[Payment]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/payment.png}
    }\\%
    \vspace*{0.05in}
    \subfloat[Shopping]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/shopping.png}
    }%
    \subfloat[Flight booking]{
      \includegraphics[width=0.28\linewidth]{img/combinedpbt/flight.png}
    }%
    \subfloat[Primitives]{\includegraphics[width=0.28\linewidth]{img/active_primitive_dist.png}\label{fig:primitivedistribution}}
    \caption{\small Comparison of PAIRED \citep{dennis2020emergent} and Flexible PAIRED with and without budget enforcing; averaged over 4 difficulty levels. (f): Percentage of active primitives over training steps.}
    \label{fig:combinedpbt}
\end{figure}

\begin{figure}[tb]
\small
    \subfloat[Difficulty level 1]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/0.png}
    }%
    \subfloat[Difficulty level 2]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/1.png}
    }%
    \subfloat[Difficulty level 3]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/2.png}
    }%
    \subfloat[Difficulty level 4]{
      \includegraphics[width=0.245\linewidth]{img/aggregatedtasks/3.png}
    }%
    \caption{\small Aggregated task success rate comparison of \WEDPb\ and baseline models on test environments with increasing difficulty levels. See Appendix \ref{ap:detailed-results} for detailed results.}
    \label{fig:tasksuccessaggregated}
    \vspace{-.7cm}
\end{figure}
We first compare the original PAIRED algorithm (which used separate antagonist and protagonist agents) to the proposed \WEDP\ algorithm that annotates the best performing agent as the antagonist.
\WEDP\ considerably improves upon PAIRED, which fails to learn in this environment (Figure \ref{fig:combinedpbt}).
One reason is that when agents are separate and have very similar rewards, especially early during training, the regret becomes very small. This uninformative signal makes it difficult for the adversary to learn.
On the other hand, Flexible PAIRED computes a consistently positive regret signal, which more clearly indicates to the adversary which environments are challenging, but still feasible. 
The further ablation studies show that adding budget improves performance for both flexible, and original PAIRED method. 

\textbf{Comparison on test environments:}
We  evaluate the performance of the proposed models and baselines on task success rate computed across test environments with different difficulty levels.
\WEDPb\ outperforms \WEDP\, indicating the budget objective significantly improves performance (Figure \ref{fig:tasksuccessaggregated}). Further, both techniques significantly outperform the baseline models on all tasks, with \WEDPb\ effectively reaching more than 80\% task success on difficulty 1 tasks.
Even as the complexity of the environments continues to increase (see Section \ref{sec:complexity}), \WEDPb\ agents still perform consistently well without degrading performance.
While CL outperforms \WEDP\ early in the training, its performance drops significantly due to ignoring agents' skill level, and making environments that are too challenging for agents to complete.
We also observe that \WEDPb\ learns faster than \WEDP\ on all environments as \WEDPb\ reacts to agents' performance faster than \WEDP{} (see Appendix \ref{ap:detailed-results}).

\label{sec:complexity}
\textbf{Environments complexity:} While agent performance improves over time, we would like to know if they are presented with more challenging environments over training.
We estimate the percentage of active primitives generated as a measure of environment complexity.
Learning a web page with more passive primitives is a relatively easier task than a page with more active primitives, because passive primitives either add noise and should ignored by the agents, or are used by agents only to navigate to another page.
On the other hand, if there are more active primitives, not only will the size of the DOM tree increase but the number of profile fields will increase, making the matching between elements and profile more challenging.
\WEDPb\ starts around 60\% random selection of primitives, and gradually generates more active primitives (Figure \ref{fig:primitivedistribution}).
Although presented with more active primitives by \WEDPb, agents are still able to improve thanks to \WEDPb's ability to accurately tune the difficulty of the environments according to agents' skill. We also observe that the distribution of the primitives shifts later in the training to more complex and relevant primitives (see Appendix \ref{ap:primitives}). 


==> WebDesignPAIRED (DeepRL Workshop) (Arxiv)/src/model.tex <==
\section{Web Environment Design}
\begin{figure}[t]
\centering
\vspace{-1.cm}
\subfloat[A \textbf{fully specified} DOM primitive where a label is created and its text is assigned.]{
  \includegraphics[width=0.28\linewidth]{img/Underspecified_DOM-2-0.pdf}
  \label{fig:underspecified0}
}
\hspace{0.15in}
\subfloat[An \textbf{underspecified} DOM tree template. The text box is always included, its text and label element are variables.]{
  \includegraphics[width=0.28\linewidth]{img/Underspecified_DOM-2-1.pdf}
  \label{fig:underspecified1}
}
\hspace{0.15in}
\subfloat[A \textbf{fully specified} DOM primitive where only the inner text within the text box is assigned.]{
  \includegraphics[width=0.28\linewidth]{img/Underspecified_DOM-2-2.pdf}
  \label{fig:underspecified2}
}
\caption{An example underspecified DOM tree template (b) and its instantiations (a,c) with different values. (*) indicates a variable; either an element or one of its attributes. (a) is used in Page 1 and (c) is used in Page 2 in Figure \ref{fig:rollout}.}
\label{fig:underspecified}
\end{figure}

We start with an empty website that is gradually populated by new pages and links between them.
Given that we represent pages by their DOM, we focus on creating DOM trees and assume links between pages are implicitly defined by events attached to certain elements.


While the most general approach to designing DOM trees would be combining a set of arbitrary elements in a bottom-up approach, this would generate a large number of malformed websites that are semantically incoherent.
Consider the second page in Figure \ref{fig:rollout} where there is a text box and a label on the top that says ``First Name''.
Now, if we have had inserted the label on top of the `Username' text box in the first page, the website would become malformed as it is ambiguous if the text box refers to `username' or `first name'.


As a result, we formulate the website design as combining a set of \textit{primitive DOM sub-trees} that are general enough to create complex websites but can be combined safely in a tree structure.
We first create a set of \textit{underspecified DOM tree templates} where certain elements and attributes are replaced with variables.
By assigning values to variables in a template, a fully specified DOM tree primitive is generated that can be combined with other primitives to create a new web page.
The order in which the primitives are combined also defines how the web page will be rendered as well.


Figure \ref{fig:underspecified} illustrates an example underspecified DOM tree template and its instantiations with different variable assignments.
We create an input template (Figure \ref{fig:underspecified1}) as a variable label and text box with a common parent.
In Figure \ref{fig:underspecified0}, we pick the label element and assign a value to its text attribute while in Figure \ref{fig:underspecified2}, we assign a value to the inner text of the text box and ignore the label element.

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{img/Adversary_rollout_and_DOM.pdf}
    \caption{\small A sample rollout of the adversary for compositional environment generation for web navigation problem. An initial observation (Obs) is given at the beginning of the rollout. $f_0$, $f_K$, $f_L$, $f_P$, and $f_I$ denote networks for encoding initial observation, generating number of pages, page indices,\protect\footnotemark primitives, and encoding LSTM inputs, respectively.}
    \label{fig:rollout}
    \vspace{-0.4cm}
\end{figure}

\footnotetext {For simplicity of illustration, we show an example generation process where primitives are generated in an increasing order of the page indices; however, in our formulation (see Section~\ref{sec:adversary} for details), the page indices corresponding to consecutive LSTM timesteps do not necessarily increase monotonically.}

\subsection{Website Design Primitives}
We introduce a new framework called gMiniWoB for automated website generation, 
which implements 40 different design primitives from 11 different underspecified DOM templates.
These primitives are widely used across the web and include `navigation bars', `product carousels', `item decks', `web forms', `item carts', `dropdowns', etc.
Every primitive includes at least one actionable element that changes the DOM structure when the agent interacts with it.
Each primitive is classified into 2 different categories based on their use in the reward computation: (i) \textbf{Active primitives (used)}, and (ii) \textbf{Passive primitives (not used)}.
$26$ of the $40$ different primitives are active primitives and the rest are passive.
When a new active primitive is added to a web page, it automatically also grows the instruction to accommodate the corresponding field.
For example, adding `First Name' text box in Figure \ref{fig:underspecified2} also adds a new field with \textit{``firstname''} key into user instruction.
This makes active primitives more complicated to learn than passive primitives, which mostly serve as noise. However, real websites contain many distracting elements (passive primitives), so it is important for agents to learn to ignore them. Appendix \ref{ap:design_primitives} details all the design primitives used, and Appendix \ref{ap:test} shows the websites in the testset.

\subsection{Adversary Architecture}
\label{sec:adversary}
We propose an autoregressive adversary policy for the compositional environment generation problem where the goal is to place a set of design primitives to a set of locations.
We parametrize the adversary with a policy $\pi_E(a^A | o^A)$ such that 
\begin{align}
    \pi_E(a^A | o^A) &= \pi(k | K)\prod_{i=0}^N{\pi(a_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k) \pi(b_i|a_{0\cdots i-1}, b_{0 \cdots i-1}, k)}
\end{align}
where $N$ is an upper limit on the number of outputs, $K$ is an upper limit on the number of locations, $a_i$ is a design primitive, $b_i$ is a location index, and $o^A$ is an initial observation.
The adversary first samples the number of locations $k$ from a parametrized Categorical distribution $Cat(0, K)$.
Conditioned on $o^A$, it executes an autoregressive model to generate a set of primitives and their corresponding locations within $[0,\cdots,k]$.

We sample $o^A$ from the standard normal distribution, similar to generative adversarial networks (GAN), to allow the adversary to diversify its design distribution.
This observation is encoded with a feed forward network $h_0=f_0(o^A)$ and $h_0$ is passed to another network $f_K$ that outputs a distribution over number of empty pages.
The same hidden state $h_0$ is passed to an LSTM network as the initial input vector and output of the LSTM is used by two independent networks $f_P$ and $f_L$ to (i) learn a distribution over design primitives and (ii) learn a distribution over locations, respectively.
We sample a primitive and a location from these distributions and they are encoded by another network $f_I$ into a hidden state which is used as the input to the LSTM at the next step.
After running for $N$ steps, sampled design actions are sent to a renderer module which generates the environment.

For the web navigation problem, $K$ denotes the number of pages in the website, locations ($b_i$) denote pages, and primitives ($a_i$) denote DOM tree primitives.
We illustrate a sample rollout of the adversary for web environment generation in Figure \ref{fig:rollout}.
We also augment the primitive design actions with a special \texttt{SKIP} action that does nothing when executed by the renderer.
This allows the adversary to control the number of primitives added.


\subsection{Flexible PAIRED}
\label{sec:flexible}
We use flexible antagonist selection to improve on the regret objective of Eq. \ref{eq:paired_regret}.
We initialize two agents $A$ and $P$. At each iteration, the adversary designs a new website and each agent collects a trajectory with return $R$ by navigating the website and the regret is:
\begin{equation}
    \textsc{REGRET} = \max \{R^A, R^P\} - 0.5 * (R^A+R^P) \label{eq:flexible_regret}
\end{equation}

This objective does not make a distinction between antagonist and protagonist agents, and instead annotates the best performing agent as the antagonist.
As long as any agent has a higher performance than the other agent, the objective will continue to improve the weakest agent.
During that time, the other agent in the policy continues learning, and therefore provide a stronger maximum performance against which we measure the regret. The Flexible PAIRED algorithm we propose is shown below. Using policy gradient updates, we train each agent in the population to optimize environmental reward, and the adversary to maximize the regret as computed in Eq. \ref{eq:flexible_regret}.

\begin{algorithm}[H]
% \SetAlgoLined
\begin{algorithmic}[1]
 \State \textbf{Input:}{$A,P$: Initialize two agents independently}
 \State $W$ $\longleftarrow$ Run the adversary $\pi_E$ to generate a new website
 \State $R^{A}$, $R^{P}$ $\longleftarrow$ Run agent $A$ and $P$ in the environment $W$ and collect rewards
 \State REGRET $\longleftarrow$ Compute regret as in Eq. \ref{eq:flexible_regret}
 \State Update adversary parameters using REGRET as the reward
 \State Update parameters of $A$ and $P$ using $R^{A}$ and $R^{P}$, respectively
\end{algorithmic}
 \caption{One step training of flexible PAIRED}
\end{algorithm}

\subsection{Budget Enforcing on Adversary}
Consider the following scenario where agents are placed on the home page of a shopping website where there are many possible elements, but only a single button that takes them to their account page.
During exploration, agents mostly collect negative rewards for taking incorrect actions, bounded to a very narrow interval (as there is only a single optimal action).
In this case, the regret is very small and non-informative, which hinders the adversary's ability to design environments at an appropriate difficulty for agents to learn.
This is true even with the proposed flexible regret objective.

To mitigate this problem, we use a budget enforcing objective in addition to the regret that binds the adversary's design budget to the performance of the best agent.
We approximate the effective budget of the adversary as the expected number of non-SKIP actions over $N$ time steps and update this budget according to whether the agents are learning.
More formally, we use the following minimization objective for budget enforcing that is added to the PAIRED objective:
\begin{equation}
    \mathcal{O}_{budget} = R^A * \sum_{i=1}^N{\log  \pi(a_i=\text{SKIP}|a_{0\cdots i-1}, b_{0,\cdots, i-1})}
\end{equation}
where $R^A$ is the reward of the antagonist (or the best-performing) agent.
This objective encourages the adversary to use less budget (more SKIP actions) when the agents are not yet learning (i.e.,  $R^A$ is negative or low); it encourages the adversary to use more budget (less SKIP actions) when the \webnav\ agents are collecting positive rewards in the environment.

==> WebDesignPAIRED (DeepRL Workshop) (Arxiv)/src/related.tex <==
\section{Related work}
Prior work on training agents to navigate the web introduced the Miniwob \citep{shi2017world} and Miniwob++ \citep{liu2018reinforcement} environments, but relied on obtaining expert demonstrations for each website, which cannot scale effectively to cover the large variety of real-world websites, and cannot adapt to changing websites. Further, these methods failed to solve complex web navigation tasks such as flight booking or social media interaction \citep{gur2018learning}. 

\citet{gur2018learning} take a step farther by training an RL agent to solve complex web navigation tasks using a scheduled curriculum. The curriculum linearly increases a parameter $p$, in which $1-p$ controls the number of web elements that are solved by querying an oracle policy, which is obtained via expert data. 
This work differs in several ways. First, we do not rely on any expert demonstrations to augment sparse rewards. We use AEG to automatically learn to generate a curriculum of web navigation tasks that are tailored to the current skill level of the agent. 
Next, we make no assumption on the availability of any website while they assume websites are given \textit{a priori}. Lastly, our web navigation agents generalize to unseen environments. 

Multi-agent training can be an effective method for automatically generating a curriculum of RL tasks (e.g. ~\citet{leibo2019autocurricula,matiisen2019teacher,graves2017automated,portelas2020teacher}). For example, Asymmetric Self Play (ASP) \citep{sukhbaatar2017intrinsic} trains two agents, in which the second agent must learn to repeat the actions taken by the first, demonstrator agent.
Both agents play in the same, fixed environment. In contrast, we use a third agent to learn to generate challenging new environments. 
POET \citep{wang2019paired,wang2020enhanced}
is an AEG technique which uses a population of adversaries to generate the terrain a 2D walker agent must learn to navigate.
To create a curriculum, POET requires generating many new environments, testing all agents within each one, and discarding environments based on a manually chosen a reward threshold, which wastes a significant amount of computation. 
\citet{campero2020learning} use a teacher to propose navigation tasks; the teacher's reward is based on whether the agent takes more steps than a threshold, a hyperparmeter that is linearly increased over the course of training.


Most closely related to our work is PAIRED \citep{dennis2020emergent}, which is an AEG method for training agents with minimal regret that works by constraining the environment-generating adversary using the performance of a second agent. However, PAIRED only demonstrated results on simple gridworld environments, and did not expand to the type of complex, high-dimensional state-action space required for web navigation. We improve on PAIRED using a more flexible estimate of the regret, as well as a budget mechanism, and show that this significantly improves performance.
